Plethysm Products, Element and Plus Constructions

Motivated by viewing categories as bimodule monoids over their isomorphism groupoids, we construct monoidal structures called plethysm products on three levels: that is for bimodules, relative bimodules and factorizable bimodules. For the bimodules, we work in the general setting of actions by categories. We give a comprehensive theory linking these levels to each other as well as to Grothendieck element constructions, indexed enrichments, decorations and algebras. Specializing to groupoid actions leads to applications including the plus construction. In this setting, the third level encompasses the known constructions of Baez-Dolan and its generalizations, as we prove. One new result is that that the plus construction can also be realized an element construction compatible with monoidal structures that we define. This allows us to prove a commutativity between element and plus constructions a special case of which was announced earlier. Specializing the results on the third level yield a criterion, when a definition of operad-like structure as a plethysm monoid -- as exemplified by operads -- is possible.

==> preamble.tex <==
%!TEX root = KMov3.tex

\usepackage{cite}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{amsmath,color}
\usepackage[v2,all]{xy}
%\usepackage{graphicx}
\usepackage{amsfonts,amssymb}
%\usepackage{mathrss,a4wide}
\usepackage{mathrsfs}
%\usepackage{eufrak}
%\usepackage{mathabx}
%\usepackage{pifont}
\usepackage{tikz}
\usetikzlibrary{cd, arrows, fit}

%\usepackage{hyperref}
\usepackage{xr-hyper}
\RequirePackage[raiselinks=false,colorlinks=true,citecolor=blue,urlcolor=black,linkcolor=blue,
bookmarksopen=true]{hyperref}
%\usepackage{graphicx}
%\newcommand{\cev}[1]{\reflectbox{\ensuremath{\vec{\reflectbox{\ensuremath{#1}}}}}}


%
%\def\maybetypo#1{\marginpar{typo? maybe}{\color{red}{\bf #1}}}  % commentary!
%\def\CHANGED#1{{\color{red}{\bf #1}}}  % commentary!
%\def\ANS#1{{\color{blue}{\bf #1}}}  % Answer!
%\def\QU#1{\marginpar{\bf Question}{\color{blue}{\bf #1}}}  % question!
\def\RMK#1{\marginpar{\color{blue}{#1}}}
%\def\CHANGED#1{}     % remove commentary!

%\usepackage[]{showkeys}
%\usepackage{refcheck}

\def\Sha{\amalg \!\!\amalg}
\usepackage{amssymb}
%\input{epsf.sty}

\usepackage{bold}
 \def\unit{\Eins}
 \def\gh{\mathbbnew{\Gamma}}
 \def\DDelta{\mathbbnew \Delta}

\catcode `\@=11
\def\numberbysection{\@addtoreset{equation}{section}
         \renewcommand{\theequation}{\thesection.\arabic{equation}}}
\numberbysection
\def\subsubsection{\@startsection{subsubsection}{3}%
  \normalparindent{.5\linespacing\@plus.7\linespacing}{-.5em}%
  {\normalfont\bfseries}}
\setcounter{tocdepth}{1}

\newtheorem{thm}{Theorem}[section]
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{claim}[thm]{Claim}
\newtheorem{dfprop}[thm]{Definition-Proposition}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{ep}[thm]{Expectation}

\theoremstyle{definition}
\newtheorem{df}[thm]{Definition}
\newtheorem{definition}[thm]{Definition}
\newtheorem{qu}[thm]{Question}
\newtheorem{rmk}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{nota}[thm]{Notation}
\newtheorem{ex}[thm]{Example}
\newtheorem{example}[thm]{Example}
\newtheorem{as}[thm]{Assumption}
\newtheorem{const}[thm]{Construction}

\def\C{\mathcal C}

\def\O{\mathcal{O}}
\def\Ab{\mathcal{A}b}
\def\Z{\mathbb{Z}}
\def\Q{\mathbb{Q}}
\def\Vect{\mathcal{V}ect}
\def\kVect{\Vect_k}
\def\dgVect{dg\mdash\kVect}
\def\cat{\mathcal{C}at}
\def\Set{\mathcal{S}et}
\def\V{\mathcal V}
\def\H{\mathscr H}
\def\E{\mathcal{E}}
\def\Mor{\mathrm{Mor}}
\newcommand{\leftsub}[2]{{\vphantom{#2}}_{#1}{#2}}


\def\SSigma{$\Sigma$}


\makeatother
\newcommand{\EZDIAG}[5]{\xymatrix
@C+=2.5cm{*+[r]{#1}
\ar@(u,l)_(0.62){\displaystyle #5}[]
\ar@<1ex>^-{#3}[r]&\ar@<1ex>^-{#4}[l]#2}}


\def\del{\partial}
\def\Coop{\check\O}
\def\id{{\mathrm{id}}}
\def\hI{\hat I}
\def\HG{\H_G}
\def\PQ{\HG}
\def\HB{\H_B}
\def\SS{\mathbb{S}}
\def\odo{\otimes \dots\otimes}
\def\cdc{\cdot \ldots\cdot}
\def\kdk{,\dots,}
\def\eps{\epsilon}
%\def\unit{1\!\!1}
\def\Hbar{{\H^{bar}}}
\def\B{\mathscr{B}}
\def\rdel{\stackrel{\leftarrow}{\del}}
\def\ldel{\stackrel{\rightarrow}{\del}}
\def\Bred{\B^{red}}
\def\nn{\nonumber}
\def\I{\mathscr {I}}
\def\J{\mathscr {J}}
\def\C{\mathscr {C}}
\def\Gr{Gr}
\def\proj{pr}
\def\Rad{\mathcal R}

\def \colim {\mathop {\rm colim}}
\def\F{\mathcal{F}}
\def\FF{\mathfrak F}
\def\asts{{\mathcal V}}
\def\ff{\mathfrak{f}}

%\def\star{{*}}
\def\stars{{\mathcal V}}
\def\clusters{{\mathcal F}}
\def\N{\mathbb{N}}
\def\dottree{\bullet\hskip-4.5pt |}
\def\simpcat{{\Delta}}


%Feynmanmacros
%\def\gh{I\hskip -3pt \Gamma}


\def\egr{\unit_{\emptyset}}
\def\nn{\nonumber}
\def\vardel{\delta}
\def\eps{\epsilon}
\def\G{\Gamma}
\def\arity{ar}
\def\Vect{\mathcal{V}ect}
%\def\dgVect{dg\Vect}
\def\dgvect{\dgVect}
\def\gVect{\Vect^{\Z}}
\def\la{\langle}
\def\ra{\rangle}
\def\Fass{{\FF}_{\it Assoc}}
\def\Flie{{\FF}_{Lie}}
\def\Fprelie{{\FF}_{pre-Lie}}
\def\CycAss{CAssoc}


\def\Graphs{{\mathcal G}\it raphs}
%\def\Gr{\Agg}
\def\GGraph{{\mathcal PR}}
\def\gg{G}
\def\Ground{({\mathcal C},\otimes)}
%\def\forget{{\mathit F}}
\def\CalC{{\mathcal C}}
\def\CalD{{\mathcal D}}
\def\CalE{{\mathcal E}}
\def\base{{B}}
\def\CalB{{\mathcal B}}
\def\CalN{{\mathcal N}}
\def\CO{{\mathcal O}}
\def\Agg{{\mathcal A}gg}
\def\Set{{\mathcal S}et}
\def\Top{{\mathcal T}op}

\def\Crl{{\mathcal C}\it rl}
\def\nCrl{\Crl_{\N}}
\def\pCrl{\Crl_{\mathrm planar}}
\def\pCyclic{\Cyclic_{\mathrm planar}}
\def\Cyclic{{\mathcal C}yc}
\def\opd{\mathcal{O}pd}
\def\CCyclic{\mathfrak  {C}}
\def\nCyclic{\Cyclic_{\N}}
\def\operads{{\mathfrak O}}
\def\props{{\mathfrak P}}
\def\properads{{\mathfrak P}^{ctd}}
\def\dioperads{{\mathfrak D}}
\def\modular{{\mathfrak M}}
\def\GGCrl{\GGraph\Crl}
\def\Coll{{\mathcal C}oll_{\GGraph,\Ground}}
\def\F{\mathcal F}
\def\FF{\mathfrak F}
\def\BB{\mathfrak B}
\def\GG{\mathfrak G}
\def\FD{\mathfrak D}
\def\Sk{{\mathcal S}k}
\def\one{1\!\!I}




\def\PF{{\mathcal P}_{\F}}
\def\FV{\F_{\V}}
\def\VV{\V_{\V}}
\def\FFV{\FF_{\V}}
\def\iV{\imath_{\V}}
\def\fL{\mathfrak{L}}


\def\R{{\mathbb R}}
\def\C{\CalC}
\def\Z{{\mathbb Z}}
\def\N{{\mathbb N}}
\def\G{\Gamma}

\def\del{\partial}
\def\colim{\mathrm{colim}}

\def\FinSet{\mathcal{F}in\mathcal{S}et}
\def\FFinSet{\mathfrak{F}in\mathfrak{S}et}
\def\surj{FS}
\def\Surj{\mathfrak{FS}}
%\def\Surj{\mathcal{S}urj}
%\def\Surj{\mathfrak{S}urj}
\def\Inj{\mathfrak{FI}}
\def\inj{FI}
\def\Int{\Inj_{*,*}}
\def\FInt{\mathfrak{I}nj_{*,*}}
\def\grep{\rho_{\Gamma}}

\def\a{\alpha}


\newcommand{\op}{\mathcal}

\def\O{{\mathcal O}}
\def\P{{\mathcal P}}
\def\Sn{{\mathbb S}_n}
\def\SS{{\mathbb S}}
\def\OS{\O_{\SS}}
\def\Snp{\SS_{n+}}
\def\Endo{{\mathcal E}nd}

\def\fSet{{\mathcal FS}et^{bij}}

\def\Op{\O^{\oplus}}
\def\sOp{s\O^{\oplus}}
\def\OSp{\O^{\oplus}_{\SS}}
\def\OSpp{\O^{\oplus}_{\SS_+}}

\def\form{\la \; ,\; \ra}
\def\Gbracket{\{\;\bullet\;\}}
\def\Liebracket{[\;\circ\;]}
\def\cLiebracket{\{\;\odot\;\}}
\def\odo{\otimes \cdots \otimes}
\def\K{\mathfrak K}
\def\crl{*}
\def\coll{col}

\def\RForest{{\mathcal RF}or}
\def\Forest{{\mathcal F}or}
\def\IOForest{{\mathcal F}or^{i/o}}
\def\Dirgraph{{\mathcal DG}}
\def\Gra{\mathfrak{G}ra}
\def\day{\circledast}

\def\wt{\mathrm{wt}}
\def\deg{\mathrm{deg}}

\def\kill{\it trun}
\def\leaf{\it leaf}

\newcommand\ccirc[2]{\, \leftsub{#1}{\circ}_{#2}}
\def\scirct{\ccirc{s}{t}}
\newcommand\Sccirc[2]{\, \leftsub{#1}{\circ}_{#2}^{S^1}}
\newcommand\mge[2]{\, \leftsub{#1}{\boxminus}_{#2}}



\newcommand{\obj}{\operatorname{Obj}}
\newcommand{\Obj}{\operatorname{Obj}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Iso}{\operatorname{Iso}}
\newcommand{\drpullback}[1][dr]{\save*!/#1-1.2pc/#1:(-1,1)@^{|-}\restore}


\newcommand{\ds}{\displaystyle}

\def\t{\tau}
\def\con{con}
%\def\{\ast}
%genop stuff
%\def\ast{{*}}
\def\V{\asts}
\def\asts{{\mathcal V}}
\def\F{\clusters}
\def\clusters{{\mathcal F}}
\def\isoclusters{Iso(\F)}
\def\Ab{{\mathcal Ab}}
\def\gAb{g\Ab}
\def\CalG{{\mathcal G}}
\def\opcat{{\mathcal O }ps}
\def\op{{\mathcal O }p}
\def\smodcat{{\mathcal M}ods}
\def\mods{\smodcat}
\def\forget{\mathit {forget}}
\def\free{\mathit {free}}
\def\T{{\mathbb T}}
\def\I{{\mathcal I}}
\def\D{\mathcal D}
\def\inthom{\underline{Hom}}

%\def\feynman{{\mathbb F}}

\def\oper{\mathcal{O}p}
\def\opers{\opcat}

\def\ta{\twoheadrightarrow}

\def\trivial{\{1\}}
\def\triv{\underline{*}}

\newcommand{\X}{{\mathcal X}}
\newcommand{\Y}{{\mathcal Y}}

\def\bl#1{\textcolor{blue}{#1}}
\def\rd#1{\textcolor{red}{#1}}
\def\mmm#1{\textcolor{magenta}{#1}}

\def\length{l}
\def\weight{wt}

%%%%%%new
\def\Bquot{\B_\Q^{quot}}
\def\Hquot{\H_\Q^{quot}}
\def\epsquot{\eps^{quot}}
\def\Deltaquot{\Delta^{quot}}
\def\etaquot{\eta^{quot}}

\def\Bred{\B^{red}}
\def\Hred{\H^{red}}
\def\epsred{\eps^{red}}
\def\Deltared{\Delta^{red}}
\def\etared{\eta^{red}}

\def\Biso{\B^{iso}}
\def\Hiso{\H^{iso}}
\def\epsiso{\eps^{iso}}
\def\Deltaiso{\Delta^{iso}}
\def\etaiso{\eta^{iso}}

%\def\Iso{\mathrm Iso}

\def\otb{\leftsub{*}\otimes_*}

\def\ops{\opcat}
\def\Fops{\F\mdash\opcat}
\def\Vmods{\V\mdash\smodcat}
\def\op{op}

\def\FFdeco{\FF_{{\it dec}\O}}

\def\mdash{\text{-}}
\def\mddash{\text{--}}
\def\un{\underline{n}}
\def\uone{\underline{1}}
\def\um{\underline{m}}

\def\ghost{\it ghost}
\def\clr{\it clr}
\def\dec{\it dec}
\def\Gpd{\mathcal{G}}
\def\M{\mathcal{M}}
\def\lab{\mathrm{lab}}
\def\bs{\boldsymbol{ \sigma}}
\def\bt{\boldsymbol{ \tau}}
%\def\be{\boldsymbol{\vec{e}}}
\newcommand\RK[1]{\marginpar{\flushleft\bl{ #1}}}
\def\io{\it io}

\def\BDelta{\Delta_{*,*}}
\def\join{\star}
\def\di{\leftsub{*}i_*}

\def\sds{(\sigma \Downarrow \sigma')}
\def\ot{\otimes}
\def\dashops{\text{-}\ops}
\def\dashopcat{\dashops}
\def\FdF{(\F\downarrow \F)}
\def\final{\mathcal{T}}
\def\Free{\it Free}
\def\IF{\Iso(\F)}
\def\el{\mathfrak{el}}
\def\GGmod{$\Gpd\mddash\Gpd$--bimodule } 
\def\GdG{\Gpd\mddash\Gpd}

\DeclareMathOperator*{\Colim}{colim}

%%%% Michaeldefs

% Comments
\newcommand\MM[1]{\marginpar{\flushleft \footnotesize \mmm{MM: #1}}}
\newcommand\defn[1]{\textbf{\emph{#1}}}

% Category conventions
%% \arbcat for Kategorie
\newcommand{\arbcat}{\mathcal{K}}
%% \G for groupoids
%% 
\newcommand{\act}{\mathcal{A}}
%% \F for Feynman categories
%% \M for monoidal categories
\newcommand{\UFC}{\mathcal{Z}}
%% \W for the isomorphism condition category
\newcommand{\W}{\mathcal{W}}
%% \Indec for the hereditary condition category
\newcommand{\Indec}{\mathcal{P}}

% UFCs
\def\Corel{\mathcal{C}orel}
\def\CCospan{\mathfrak{C}ospan}
\def\Cospan{\mathcal{C}ospan}
\def\SSpan{\mathfrak{S}pan}
\def\Span{\mathcal{S}pan}

% Plethysm products
\newcommand{\pl}{\mathbin{\square}}
\newcommand{\epl}{\diamond}
\newcommand{\bepl}{\mathbin{(\diamond)}}
% \newcommand{\hp}{\mathbin{\hat \otimes}}

% Biaction
\newcommand{\biact}{\mid}

% Other
\DeclareMathOperator{\Fun}{Fun}
\DeclareMathOperator{\Lan}{Lan}
\DeclareMathOperator{\Ind}{Ind}

% tikz stuff
\tikzstyle{none}=[]
\tikzstyle{Vertex}=[fill=white, draw=black, shape=circle]
\tikzstyle{Hyperedge}=[fill=black, draw=black, shape=circle,inner sep=0.6mm]
\tikzstyle{White}=[fill=white, draw=black, shape=circle]
\tikzstyle{Black}=[fill=black, draw=black, shape=circle]
\tikzstyle{WhiteSq}=[fill=white, draw=black, shape=rectangle]
\tikzstyle{BlackSq}=[fill=black, draw=black, shape=rectangle]
\tikzstyle{Red}=[fill=red, draw=black, shape=circle]
\tikzstyle{Blue}=[fill=blue, draw=black, shape=circle]

\tikzstyle{Arrow}=[->]
\tikzstyle{Mapsto}=[{|->}]
\tikzstyle{Dash}=[-, dashed]
\tikzstyle{DashArrow}=[->, dashed]
\tikzstyle{Double}=[<->]

% Font
\usepackage{enumitem}
\setlist[description]{font=\normalfont\scshape}


%%% plus construction macros %%%

% Plus construction for categories
\newcommand{\catplus}[1]{\mathcal{P}l({#1})}
\newcommand{\catplusp}[1]{\mathcal{P}l^{u}({#1})}
\newcommand{\catplusg}[1]{\mathcal{P}l^{c}({#1})}
\newcommand{\catplusgp}[1]{\mathcal{P}l^{uc}({#1})}
\newcommand{\catplusgcp}[1]{\mathcal{P}l^{\it gcp}({#1})}
\newcommand{\catplushyp}[1]{\mathcal{P}l^{\it hyp}({#1})}

% NC plus construction
\newcommand{\monplus}[1]{\mathcal{P}l_{\otimes}({#1})}
\newcommand{\monplusp}[1]{\mathcal{P}l_{\otimes}^{u}({#1})}
\newcommand{\monplusg}[1]{\mathcal{P}l_{\otimes}^{c}({#1})}
\newcommand{\monplusgp}[1]{\mathcal{P}l_{\otimes}^{uc}({#1})}
\newcommand{\monplusgr}[1]{\mathcal{P}l_{\otimes}^{graph}({#1})}
\newcommand{\monplusgcp}[1]{\mathcal{P}l_{\otimes}^{\it gcp}({#1})}
\newcommand{\monplusgcpgr}[1]{\mathcal{P}l_{\otimes}^{\it graph, gcp}({#1})}
\newcommand{\monplushyp}[1]{\mathcal{P}l_{\otimes}^{\it hyp}({#1})}
\newcommand{\monplushypgr}[1]{\mathcal{P}l_{\otimes}^{\it graph, hyp}({#1})}

% Localized plus construction
\newcommand{\locmonplus}[1]{\mathcal{P}l_{\otimes}({#1})_{loc}}
\newcommand{\locmonplusp}[1]{\mathcal{P}l_{\otimes}^{u}({#1})_{loc}}
\newcommand{\locmonplusg}[1]{\mathcal{P}l_{\otimes}^{c}({#1})_{loc}}
\newcommand{\locmonplusgp}[1]{\mathcal{P}l_{\otimes}^{uc}({#1})_{loc}}
\newcommand{\locmonplusgcp}[1]{\mathcal{P}l_{\otimes}^{\it gcp}({#1})_{loc}}
\newcommand{\locmonplushyp}[1]{\mathcal{P}l_{\otimes}^{\it hyp}({#1})_{loc}}

%Reduced
\newcommand{\redmonplus}[1]{\mathcal{P}l_{\otimes}({#1})_{red}}
\newcommand{\redmonplusp}[1]{\mathcal{P}l_{\otimes}^{u}({#1})_{red}}
\newcommand{\redmonplusg}[1]{\mathcal{P}l_{\otimes}^{c}({#1})_{red}}
\newcommand{\redmonplusgp}[1]{\mathcal{P}l_{\otimes}^{uc}({#1})_{red}}
\newcommand{\redmonplusgcp}[1]{\mathcal{P}l_{\otimes}^{\it gcp}({#1})_{red}}
\newcommand{\redmonplushyp}[1]{\mathcal{P}l_{\otimes}^{\it hyp}({#1})_{red}}

% Alias for reduced plus construction
\newcommand{\plus}[1]{{#1}^+}
\newcommand{\plusp}[1]{{#1}^{+, \it u}}
\newcommand{\plusg}[1]{{#1}^{+, \it c}}
\newcommand{\pluspg}[1]{{#1}^{+, \it uc}}
\newcommand{\plusgr}[1]{{#1}^{+, \it graph}}
\newcommand{\plusgcp}[1]{{#1}^{+, \it gcp}}
\newcommand{\plusgcpgr}[1]{{#1}^{+, \it graph, gcp}}
\newcommand{\plushyp}[1]{{#1}^{+, \it hyp}}
\newcommand{\plushypgr}[1]{{#1}^{+, \it graph, hyp}}

% Generic
\newcommand{\anyplus}{\mathcal{P}_+}
\newcommand{\anyplusp}{\anyplus^{u}}
\newcommand{\anyplusg}{\anyplus^{c}}
\newcommand{\anyplusgp}{\anyplus^{uc}}
\newcommand{\anyplusgcp}{\anyplus^{gcp}}
\newcommand{\anyplushyp}{\anyplus^{hyp}}

% Graphical plus constructions
\newcommand{\gplus}[1]{\mathcal{G}r({#1})}
\newcommand{\gplusp}[1]{\mathcal{G}r^{p}({#1})}
\newcommand{\gplusgcp}[1]{\mathcal{G}r^{gpd}({#1})}
\newcommand{\gplushyp}[1]{\mathcal{G}r^{hyp}({#1})}

%Graphical nc plus constructions
\newcommand{\mongplus}[1]{\mathcal{G}r_{\otimes}({#1})}
\newcommand{\mongplusgcp}[1]{\mathcal{G}r_{\otimes}^{gpd}({#1})}
\newcommand{\mongplusp}[1]{\mathcal{G}r_{\otimes}^{p}({#1})}
\newcommand{\mongplushyp}[1]{\mathcal{G}r_{\otimes}^{hyp}({#1})}

